The Finite Element Immersed Boundary Method with Distributed Lagrange multiplier

We introduce a new formulation for the finite element immersed boundary method which makes use of a distributed Lagrange multiplier. We prove that a full discretization of our model, based on a semi-implicit time advancing scheme, is unconditionally stable with respect to the time step size.

==> tables/dlm_inf_sup.tex <==
\begin{tabular}{cc c c c c c c c c c c c c}
\toprule
\multicolumn{13}{c}{Codimension one.} \\
\midrule
 & &\multicolumn{11}{c}{$h_x$} \\
$h_s$ & &$\frac{ 1}{48}$ & &$\frac{ 1}{40}$ & &$\frac{ 1}{32}$ & &$\frac{ 1}{24}$ & &$\frac{ 1}{16}$ & &$\frac{1}{8}$ \\ \midrule
$1/48$ & & \cellcolor{color0}1.026 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/40$ & & \cellcolor{color0}1.026 & & \cellcolor{color0}1.024 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/32$ & & \cellcolor{color0}1.026 & & \cellcolor{color0}1.024 & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.019 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/24$ & & \cellcolor{color0}1.026 & & \cellcolor{color0}1.024 & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.017 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/16$ & & \cellcolor{color0}1.026 & & \cellcolor{color0}1.024 & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.017 & & \cellcolor{color0}1.010 & & \cellcolor{color9}inf-sup \\ \midrule
$1/8$ & & \cellcolor{color0}1.026 & & \cellcolor{color0}1.024 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.017 & & \cellcolor{color0}1.009 & & \cellcolor{color0}0.987 \\ \midrule
\multicolumn{13}{c}{Codimension zero.} \\
\midrule
$1/48$ & & \cellcolor{color0}0.996 & & \cellcolor{color0}0.995 & & \cellcolor{color0}0.995 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/40$ & & \cellcolor{color0}0.995 & & \cellcolor{color0}0.995 & & \cellcolor{color0}0.995 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/32$ & & \cellcolor{color0}0.992 & & \cellcolor{color0}0.992 & & \cellcolor{color0}0.992 & & \cellcolor{color0}0.992 & & \cellcolor{color0}0.991 & & \cellcolor{color9}inf-sup \\ \midrule
$1/24$ & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.993 & & \cellcolor{color9}inf-sup & & \cellcolor{color9}inf-sup \\ \midrule
$1/16$ & & \cellcolor{color0}0.993 & & \cellcolor{color0}0.991 & & \cellcolor{color0}0.988 & & \cellcolor{color0}0.986 & & \cellcolor{color0}0.985 & & \cellcolor{color0}0.987 \\ \midrule
$1/8$ & & \cellcolor{color0}0.996 & & \cellcolor{color0}0.995 & & \cellcolor{color0}0.992 & & \cellcolor{color0}0.987 & & \cellcolor{color0}0.974 & & \cellcolor{color0}0.977 \\ \bottomrule
\end{tabular}

==> tables/fsi_cfl.tex <==
%\usepackage{color,colortbl}
%\usepackage{booktabs}
%\definecolor{color0}{rgb}{0.4,1.0,0.4}
%\definecolor{color1}{rgb}{1.0,1.0,0.4}
%\definecolor{color2}{rgb}{1.0,1.0,0.4}
%\definecolor{color3}{rgb}{1.0,0.501960784314,0.0}
%\definecolor{color4}{rgb}{1.0,0.501960784314,0.0}
%\definecolor{color5}{rgb}{1.0,0.0,0.0}
%\definecolor{color6}{rgb}{1.0,0.0,0.0}
%\definecolor{color7}{rgb}{1.0,0.0,0.0}
%\definecolor{color8}{rgb}{1.0,0.0,0.0}
%\definecolor{color9}{rgb}{1.0,0.0,0.0}
\begin{tabular}{ c c c c c c c c c c cc cc cc cc}\toprule
\multicolumn{17}{c}{Structure mesh size $h_s$} \\ \cmidrule{3-17}
 & &\multicolumn{7}{c}{\textsc{fe-ibm} codimension one.} & & \multicolumn{7}{c}{\textsc{fe-ibm} codimension zero.}\\
 \cmidrule{1-1}\cmidrule{3-9}\cmidrule{11-17}
$\Delta t$ & &$\frac{ 1}{32}$ & &$\frac{ 1}{24}$ & &$\frac{ 1}{16}$ & &$\frac{1}{8}$ 
& &$\frac{ 1}{32}$ & &$\frac{ 1}{24}$ & &$\frac{ 1}{16}$ & &$\frac{1}{8}$
\\ \cmidrule{1-1}\cmidrule{3-9}\cmidrule{11-17}
$1\cdot 10^{-2}$ & & \cellcolor{color1}0.941 & & \cellcolor{color1}0.941 & & \cellcolor{color1}0.941 & & \cellcolor{color1}0.940 
& & \cellcolor{color1}0.949 & & \cellcolor{color1}0.949 & & \cellcolor{color1}0.949 & & \cellcolor{color1}0.948 \\
$2\cdot 10^{-2}$ & & \cellcolor{color1}0.941 & & \cellcolor{color1}0.940 & & \cellcolor{color1}0.940 & & \cellcolor{color1}0.940 
& & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 \\
$3\cdot 10^{-2}$ & & \cellcolor{color1}0.941 & & \cellcolor{color1}0.940 & & \cellcolor{color1}0.940 & & \cellcolor{color1}0.939 
& & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.947 \\
$5\cdot 10^{-2}$ & & \cellcolor{color9}\textsc{cfl} & & \cellcolor{color1}0.940 & & \cellcolor{color1}0.939 & & \cellcolor{color1}0.938 
& & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 \\
$1\cdot 10^{-1}$ & & \cellcolor{color9}\textsc{cfl} & & \cellcolor{color9}\textsc{cfl} & & \cellcolor{color8}\textsc{cfl} & & \cellcolor{color1}0.936
& & \cellcolor{color1}0.945 & & \cellcolor{color1}0.945 & & \cellcolor{color1}0.945 & & \cellcolor{color1}0.944 \\
\cmidrule{1-1}\cmidrule{3-9}\cmidrule{11-17}
% & &\multicolumn{7}{c}{\textsc{ibm-dlm} codimension one.} & & \multicolumn{7}{c}{\textsc{ibm-dlm} codimension zero.}\\ \cmidrule{1-1}\cmidrule{3-9}\cmidrule{11-17}
 $\Delta t$ & &$\frac{ 1}{32}$ & &$\frac{ 1}{24}$ & &$\frac{ 1}{16}$ & &$\frac{1}{8}$ 
& &$\frac{ 1}{32}$ & &$\frac{ 1}{24}$ & &$\frac{ 1}{16}$ & &$\frac{1}{8}$
\\ \cmidrule{1-1}\cmidrule{3-9}\cmidrule{11-17}
$1\cdot 10^{-2}$ & & \cellcolor{color0}1.023 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.023 
& & \cellcolor{color0}0.993 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.989 & & \cellcolor{color0}0.994 \\ 
$2\cdot 10^{-2}$ & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 
& & \cellcolor{color0}0.992 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.989 & & \cellcolor{color0}0.993 \\
$3\cdot 10^{-2}$ & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 & & \cellcolor{color0}1.022 
& & \cellcolor{color0}0.992 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.989 & & \cellcolor{color0}0.993 \\
$5\cdot 10^{-2}$ & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.021 & & \cellcolor{color0}1.022 
& & \cellcolor{color0}0.992 & & \cellcolor{color0}0.994 & & \cellcolor{color0}0.988 & & \cellcolor{color0}0.992 \\ 
$1\cdot 10^{-1}$ & & \cellcolor{color0}1.020 & & \cellcolor{color0}1.020 & & \cellcolor{color0}1.020 & & \cellcolor{color0}1.020 
& & \cellcolor{color0}0.991 & & \cellcolor{color0}0.993 & & \cellcolor{color0}0.987 & & \cellcolor{color0}0.991 \\ \bottomrule

%\multicolumn{9}{c}{\feibm codimension zero.} \\ \midrule
%%%%%$1\cdot 10^{-2}$ & & \cellcolor{color1}0.949 & & \cellcolor{color1}0.949 & & \cellcolor{color1}0.949 & & \cellcolor{color1}0.948 \\ \midrule
%%%%%$2\cdot 10^{-2}$ & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 \\ \midrule
%%%%%$3\cdot 10^{-2}$ & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.948 & & \cellcolor{color1}0.947 \\ \midrule
%%%%%$5\cdot 10^{-2}$ & & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 & & \cellcolor{color1}0.947 \\ \midrule
%%%%%$1\cdot 10^{-1}$ & & \cellcolor{color1}0.945 & & \cellcolor{color1}0.945 & & \cellcolor{color1}0.945 & & \cellcolor{color1}0.944 \\ \midrule
%\multicolumn{9}{c}{\ibmdlm codimension zero.} \\ \midrule
%$1\cdot 10^{-2}$ 
%$2\cdot 10^{-2}$ 
%$3\cdot 10^{-2}$ 
%$5\cdot 10^{-2}$ 
%$1\cdot 10^{-1}$ 
\end{tabular}

